Serving Recurrent Neural Networks Efficiently with a Spatial Accelerator

Recurrent Neural Network (RNN) applications form a major class of AI-powered, low-latency data center workloads. Most execution models for RNN acceleration break computation graphs into BLAS kernels, which lead to significant inter-kernel data movement and resource underutilization. We show that by supporting more general loop constructs that capture design parameters in accelerators, it is possible to improve resource utilization using cross-kernel optimization without sacrificing programmability. Such abstraction level enables a design space search that can lead to efficient usage of on-chip resources on a spatial architecture across a range of problem sizes. We evaluate our optimization strategy on such abstraction with DeepBench using a configurable spatial accelerator. We demonstrate that this implementation provides a geometric speedup of 30x in performance, 1.6x in area, and 2x in power efficiency compared to a Tesla V100 GPU, and a geometric speedup of 2x compared to Microsoft Brainwave implementation on a Stratix 10 FPGA.

==> Makefile <==
PAPER = main
TEX = $(wildcard *.tex text/*.tex)
BIB = references.bib
FIGS = $(wildcard figs/*.pdf figs/*.png graphs/*.pdf graphs/*.png)
CODE = $(wildcard code/*)

.PHONY: all export clean

$(PAPER).pdf: $(TEX) $(BIB) $(FIGS) $(CODE)
	echo $(FIGS)
	pdflatex $(PAPER)
	bibtex $(PAPER)
	pdflatex $(PAPER)
	pdflatex $(PAPER)
	#cp main.pdf ~/Dropbox/SYSML_RNN_DRAFT/

lunch: $(PAPER).pdf
	bash publish.sh $(PAPER).pdf

test: $(TEX) $(BIB) $(FIGS)
	echo $(FIGS)
	pdflatex $(PAPER)
	bibtex $(PAPER)
	pdflatex $(PAPER)
	pdflatex $(PAPER)

continuous:
	latexmk -pdf -pvc -halt-on-error main

# figs/speedupbars.tex: figs/speedupbars.gp figs/speedupbars.dat
# 	cd figs && gnuplot speedupbars.gp
# 	cd figs && sed -i.bak 's/speedupbars/figs\/speedupbars/' speedupbars.tex

clean:
	rm -f *.aux *.bbl *.blg *.log *.out $(PAPER).pdf



==> code/gemm.tex <==
\begin{figure}
\centering

\newsavebox{\gemm}
\begin{lrbox}{\gemm}
\begin{lstlisting}[language=scala,linewidth=0.91\columnwidth]
// Custom floating point format
// 11 mantissa, 5 exponent bits
type Half = FltPt[11,5]

def main(args: Array[String]) {

  // Load data from files
  val a: Matrix[Half] = loadMatrix[Half](args(0))
  val b: Matrix[Half] = loadMatrix[Half](args(1))

  // Allocate space on accelerator DRAM
  val A = DRAM[Half](a.rows,a.cols)
  val B = DRAM[Half](b.rows,b.cols)
  val C = DRAM[Half](a.rows,b.cols)

  // Create explicit design parameters
  val M = 128 (64, 1024)  // Tile size for output rows
  val N = 128 (64, 1024)  // Tile size for output cols
  val P = 128 (64, 1024)  // Tile size for common
  val PAR_K  = 2 (1, 8)   // Unroll factor of k 
  val PAR_J  = 2 (1, 16)  // Unroll factor of j

  // Transfer data to accelerator DRAM
  sendMatrix(A, a)
  sendMatrix(B, b)

  // Specify the accelerator design
  Accel {
    // Produce C in M x N tiles
    Foreach(A.rows by M, B.cols by N){ (ii,jj) =>
      val tileC = SRAM[Half](M, N)
      
      // Combine intermediates across common dimension
      MemReduce(tileC)(A.cols by P){ kk =>
        // Allocate on-chip scratchpads
        val tileA = SRAM[Half](M, P) 
        val tileB = SRAM[Half](P, N)
        val accum = SRAM[Half](M, N)
          
        // Load tiles of A and B from DRAM
        tileA load A(ii::ii+M, kk::kk+P)  // M x P
        tileB load B(kk::kk+P, jj::jj+N)  // P x N
        
        // Combine intermediates across a chunk of P
        MemReduce(accum)(P by 1 par PAR_K){ k =>
          val partC = SRAM[Half](M, N)
          Foreach(M by 1, N by 1 par PAR_J){ (i,j) =>
            partC(i,j) = tileA(i,k) * tileB(k,j)
          }
          partC
        // Combine intermediates with element-wise add
        }{(a,b) => a + b }
      }{(a,b) => a + b }

      // Store the tile of C to DRAM
      C(ii::ii+M, jj::jj+N) store tileC
    }
  }

  // Save the result to another file
  saveMatrix(args(2), getMatrix(C))
}
\end{lstlisting}
\end{lrbox}

\begin{tabular}{m{0.01cm} l} & \usebox{\gemm} \end{tabular}
\caption{Basic matrix multiplication ($C$~=~$A\cdot B$) implemented in Spatial with language
constructs from Table~\ref{t:syntaxTable}
\vspace{-10pt}}
\label{fig:matmult}
\end{figure}  

